Reasoning Through Memorization: Nearest Neighbor Knowledge Graph Embeddings

Previous knowledge graph embedding approaches usually map entities to representations and utilize score functions to predict the target entities, yet they typically struggle to reason rare or emerging unseen entities. In this paper, we propose kNN-KGE, a new knowledge graph embedding approach with pre-trained language models, by linearly interpolating its entity distribution with k-nearest neighbors. We compute the nearest neighbors based on the distance in the entity embedding space from the knowledge store. Our approach can allow rare or emerging entities to be memorized explicitly rather than implicitly in model parameters. Experimental results demonstrate that our approach can improve inductive and transductive link prediction results and yield better performance for low-resource settings with only a few triples, which might be easier to reason via explicit memory. Code is available at https://github.com/zjunlp/KNN-KG.

==> charts/dataset.tex <==
\let\mc\multicolumn
\begin{table}[t]
\caption{Statistics of datasets used in the link prediction task under transductive and inductive settings.}
\centering
\resizebox{1.0\textwidth}{!}{% <------ Don't forget this %
\begin{tabular}{lcccc}
\toprule
          & \mc{2}{c}{WN18RR}             &              \mc{2}{c}{FB15k-237}              \\
           \cmidrule(lr){2-3}                        \cmidrule(lr){4-5}              
          &     Transductive &  Inductive & Transductive &  Inductive \\
\midrule
Relations & \mc{2}{c}{11}        & \mc{2}{c}{237}                                     \\
\midrule
          &         \mc{4}{c}{Training}                                            \\
                \cmidrule(lr){2-5}                        
Entities  & 40,943 &    32,755 &    14,541 &    11,633                               \\
Triples   & 86,835 &    69,585 &    272,115 &   215,082             \\
\midrule
          &        \mc{4}{c}{Validation}             \\
                 \cmidrule(lr){2-5}            
Entities  & -   & 4,094 & - &  1,454 \\
Triples   & 3,034 & 11,381    & 17,535 &    42,164      \\
\midrule
          &        \mc{4}{c}{Test}                    \\
              \cmidrule(lr){2-5}            
Entities  & -       & 4,094     &   -  & 1,454      \\
Triples   & 3,134   & 12,087    & 20,466&52,870       \\
\bottomrule
\end{tabular}%
}
\label{tb:dataset}
\end{table}

==> charts/knowledge_store.tex <==
\begin{table}[!htb]

\centering
\caption{Statistics of knowledge store built on two datasets, radio of retrieved entity embeddings from two resources, and inference time per query triple.}
\resizebox{0.7\textwidth}{!}{
\begin{tabular}{lccccc}
\toprule
KG  & memory & from $\mathcal{D}$ & from $\mathcal{T}$  & retrieved $\mathcal{D}/\mathcal{T}$ (\%) & time \\
\midrule
WN18RR          & 509M   & 40,943 & 139,170  & 13/87  & 7.75ms             \\
FB15k-237       & 1671M  & 14,541 & 544,230 &  4/96  &       13.6ms      \\
\bottomrule
\end{tabular}
}

\label{tb:knowledge_store}
\end{table}

==> figs/diff_plms.tex <==
\begin{figure}
    \centering
    \includegraphics[scale=0.5]{figs/diff_plms.pdf}
    \caption{Effect of different PLMs (BERT, RoBERTa, SpanBERT) on FB15k-237 dataset.}
    \label{fig:diff_plms}
\end{figure}


==> figs/intro_figure.tex <==
\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.50\textwidth]{figs/intro.pdf}
    \caption{Our model not only use its mind (MLM head) but also retrieve the entity from the knowledge store constructed by the descriptions and the triples.}
    \label{fig:intro}
\end{figure}

==> figs/k_lambda.tex <==

\begin{figure}[htbp]
%   \begin{minipage}[t]{0.425\linewidth}
    \centering
    \includegraphics[scale=0.4]{figs/k_result.pdf}
    \caption{Effect of the number of neighbors from knowledge store.}
    \label{fig:topk}
%   \end{minipage}%
%   \hspace{0.05\linewidth}
%   \begin{minipage}[t]{0.425\linewidth}
    
%   \end{minipage}
\end{figure}


\begin{figure}
    \centering
    \includegraphics[scale=0.4]{figs/lambda_result.pdf}
    \caption{Effect of interpolation parameter $\lambda$ on FB15k-237 dataset.}
    \label{fig:lambda}
\end{figure}


==> figs/model.tex <==


\begin{figure*}[!htbp] %H为当前位置，!htb为忽略美学标准，htbp为浮动图形
\centering %图片居中
\includegraphics[width=0.98\textwidth]{./figs/main.pdf} %插入图片，[]中设置图片大小，{}中是图片文件名
\caption{Entity Vocabulary Expansion (Figure a), Masked Entity Modeling (Figure b), and Knowledge Store Construction from entity de build method based on two subsections (Figure c). 
Entities in color will be encoded into contextualized entity representation and added into our knowledge store.
Examples are taken from \protect\cite{liu2021indigo}. }
\label{fig:model}
\end{figure*}


